On the Resilience of RTL NN Accelerators: Fault Characterization and Mitigation

Machine Learning (ML) is making a strong resurgence in tune with the massive generation of unstructured data which in turn requires massive computational resources. Due to the inherently compute- and power-intensive structure of Neural Networks (NNs), hardware accelerators emerge as a promising solution. However, with technology node scaling below 10nm, hardware accelerators become more susceptible to faults, which in turn can impact the NN accuracy. In this paper, we study the resilience aspects of Register-Transfer Level (RTL) model of NN accelerators, in particular, fault characterization and mitigation. By following a High-Level Synthesis (HLS) approach, first, we characterize the vulnerability of various components of RTL NN. We observed that the severity of faults depends on both i) application-level specifications, i.e., NN data (inputs, weights, or intermediate), NN layers, and NN activation functions, and ii) architectural-level specifications, i.e., data representation model and the parallelism degree of the underlying accelerator. Second, motivated by characterization results, we present a low-overhead fault mitigation technique that can efficiently correct bit flips, by 47.3% better than state-of-the-art methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> chapters/11-acknowledgement.tex <==
\section{Acknowledgment}
%This work was sponsored in part by Defense Advanced Research Projects Agency (DARPA) under contract \#HR0011-13-C-0022. The views expressed are those of the authors and do not reflect the official policy or position of the Department of Defense or the U.S. Government.
The research leading to these results has received funding from the Ministry of Economy and Competitiveness of Spain under contract number TIN2015-65316-p.

==> chapters/4-RTLDescription.tex <==
\section{RTL Design of the DNN and Fault Injection Unit}
\label{sec:model}
We elaborate the RTL design of the DNN and fault injection unit in Sections \ref{RTL:1} and \ref{RTL:2}, respectively.
\subsection{The Overall Architecture of the RTL Design}
\label{RTL:1}
In this paper, we consider the most common features of state-of-the-art FPGA- \cite{li2016high}, \cite{Nurvitadhi2017}, \cite{Zhang2017}, \cite{Lu2017} and ASIC-based \cite{tpu} DNN accelerators and accordingly adapt our RTL design. Note that the RTL design design can be potentially synthesized on the FPGA or ASIC. Below, we detail the adapted features:
\begin{itemize}
\item \textbf{Storage Elements}: In DNN acceleration platforms, off- and on-chip memories are exploited to accommodate various types of data. Off-chip memory (usually DRAM-based) has a large size, low bandwidth, and it is suitable to accommodate large volumes of input data. In contrast, on-chip memory (usually SRAM-based in ASIC or Block RAM in FPGA) has a small size, distributed architecture, high bandwidth, and it is used to cope with the weights of the DNN. These memories are implemented in our RTL model using an HLS tool and with the following structure: an off-chip memory with a bandwidth of 512 bits/cycle (similar to DDR-3 \cite{ddr}) and a set of 64 distributed on-chip memories, 32 kb each (similar to BRAM \cite{bram}).
\item \textbf{Processing Elements ($PE$)}: The architecture of the DNN is inherently parallel and can be efficiently mapped into massively parallel processing fabrics. Toward this goal, computational hardware blocks in ASICs (64K 8-bits fixed-point custom processing elements in Google TPU \cite{tpu}) or Digital Signal Processing (DSP) units in FPGAs (few hundreds) can be exploited. In our RTL design, we use 64 fixed-point $PE$s in parallel. Note that as seen in the part \encircle{3} of Figure \ref{fig:overall}, our $PE$s are multipliers-adders that enable us to perform the matrix multiplications, as the core computational unit of the DNN computation.  
\item \textbf{Execution Model}: Compared to control-flow based hardware such as general-purpose processors, ASICs/FPGAs typically utilize data streaming execution model, which is the key advantage to achieve the significant throughput. This model is considered in our design, as well. 
\end{itemize}
  
Furthermore, to amortize access costs to the emulated off-chip memory by efficiently reusing already-loaded data, we modify the conventional matrix multiplication algorithm. We perform the matrix multiplication column-by-column, instead of the conventional row-by-row approach. Accordingly, with respect to the structure of our RTL design and for a DNN classifier with $N_l$ layers, we can compute the total number of cycles to classify a single input data record ($T$) using the Equation \ref{T}. Among layers, $L_0$ is the input, $L_{N_l-1}$ is the output, and the rest are hidden layer(s). Also, $|L_i|$ indicates the size of the layer $i$, which equals to number of neurons. $T$ equals to the total number of operations within the classification divided by the number of $PE$s. Note that the computation of the activation function does not incur any additional clock cycle, since it is modeled as a combinational circuit. 
\begin{equation}
\label{T}
T = \frac{\sum_{i=0}^{N_l-2} {|L_i| * |L_{i+1}|}}{\#PEs}
\end{equation} 

%We elaborate it for an example as shown in Figure \ref{fig:matrix}. In this figure, $H_0$ is the weight matrix that is located in on-chip memories and \textit{I} is the input dataset matrix that is located in the off-chip memory. \textit{B} is the bandwidth of the off-chip memory (in this example, B = 2 data/cycle)\footnote{In our development, we emulate a DDR-3 bandwidth, which is 512 bits/cycle \cite{ddr}.}. Also, the number of parallel elements ($P$) is assumed to be 4. As it can be seen, we perform the matrix multiplication column-by-column, by leveraging blocking and by reusing the already-loaded data from off-chip memory (instead of the common row-by-row multiplication approach). Following this approach, we only need  $\frac{|I|}{B}$ memory accesses. Furthermore, $P$= 4 leads to 4 operations per cycle. Consequently, considering the streaming fashion of computations, the required number of cycles to perform the correspondent matrix multiplication can be computed as $\frac{|H_0|*|I|}{P}$.
 
%Thanks to the aforementioned approach, for a general DNN classifier, we can compute the total number of cycles to classify a single input data record ($T$), as shown in Equation \ref{T}. The number of operations (cycles) equals to "the aggregation of number of operations per layer" divided by $P$. We assume that DNN has $N_l$ layers in total, i.e., $\{L_0, L_1, ..., L_{N_l-1}\}$, where $L_0$ is the input layer, $L_{N_l-1}$ is the output layer, and the rest are hidden layers of DNN. $|L_i|$ indicates the size of the layer $i$, which equals to number of neurons. 
%\begin{equation}
%\label{T}
%T = \frac{\sum_{i=0}^{N_l-2} {|L_i| * |L_{i+1}|}}{P}
%\end{equation} 

%figure
%\begin{figure}
%\centering
%\includegraphics[width=8cm]{images/matrix_multiplier.pdf} %, height=5cm
%\caption{An optimized parallel matrix multiplication approach, while the off-chip memory accesses are %minimized.}
%\label{fig:matrix}
%\end{figure}

\subsection{Fault Injection Unit}
\label{RTL:2}
The fault injection unit is developed on top of the RTL design of the DNN classifier. Faults are injected into registers in the data-path of processing units. Registers are the main state-holding elements in the processing pipeline of the RTL design. There are three types of registers in our design, i.e., input registers (\textit{IR}s), weight registers (\textit{WR}s), and intermediate registers (\textit{IMR}s), which are leveraged to latch input, weights, and intermediate data, respectively. The total number of bits, which can be potentially corrupted, can be computed using Equation \ref{S}, where $numR_i$ and $sizeR_i$ represent the number and size (bit-width) of register type $i \in \{IR, WR, IMR\}$, respectively.
\begin{equation}
\label{S}
S = \sum_{i \in \{IR, WR, IMR\}}{numR_i * sizeR_i}
\end{equation}  

\subsubsection{\textbf{When}, \textbf{\textit{Where}}, and \textbf{\textit{How frequently}} are Faults Injected?}
Our fault injection unit supports permanent (stuck-at-0 and stuck-at-1) and transient faults. Permanent faults can cause bits to permanently get stuck at 0 or 1. Thus, they result in a bit flip, if and only if the logical value of the faulty bit is different than the value at which the physical bit is stuck. In contrast, transient faults flip contents of bits for a few cycles (typically one cycle). In both cases, we assume that faults are confined to a single register. In short, we consider the following: 
\begin{itemize}
\item \textit{\textbf{When?}} Permanent faults are stuck at 0 or 1 for the whole classification cycles, from first to the last. In contrast, transient faults occur in a single random cycle within classification cycles.
\item \textit{\textbf{Where?}} We inject faults into a set of bits of a single register of the RTL design of the DNN. The register and bits to be corrupted are randomly selected.
\item \textit{\textbf{How frequently?}} To comprehensively study the impact of faults in the classification error, we repeat the fault injection for each input data item (for instance, for each image in the image classification case). In other words, we generate a fault and while input data is streaming into the classifier one-by-one, we inject the generated fault for each of the input data items, individually. This is an artificially high fault rate, but allows us to quickly evaluate the impact of faults on the DNN.
\end{itemize}

We use pseudorandom number generation libraries of Bluespec to simulate the fault generation campaigns, by selecting a random register, set of bits, and cycle (in the transient case). Later on, we inject the generated fault in the corresponding locations/cycles, while streaming the input data into the classifier, allow the completion of the classification for all input data, and finally, compute the classification error by comparing classified against the golden output data provided by the benchmark suite. To achieve statistically significant results, we repeat experiments several times. Each time a different fault (set of bits, register, and cycle) is randomly generated and injected, while the whole input data is streamed again. Finally, after repeating the injection a statistically significant number of times, the final classification error is calculated as the average error of all trials. We elaborate our statistical fault injection methodology in Section \ref{sec:statis}.%, where we experimentally determine the statistically significant number of trials.   

\subsubsection{Statistical Fault Injection Methodology} 
\label{sec:statis}
The number of possibilities for the fault injection is directly related to $S$ and $S * T$, for permanent and transient cases, respectively (As defined in Equations \ref{T} and \ref{S}, $T$ is the total number of classification cycles and $S$ is the total number of bits to be corrupted.). More specifically, for our DNN model with the baseline configuration introduced in Section \ref{sec1}, $S$= 4969 and $S * T$= 7890772. Due to large number of possibilities, it is almost impossible to compute the vulnerability of the design in a reasonable time by following the aforementioned deterministic solution. To alleviate this problem and as an alternative solution, we follow a statistical fault injection approach \cite{Leveugle2009}, where only a subset of possible faults is injected by repeating the trials. This subset is randomly selected with respect to the target injection bits ($S$) and clock cycles ($T$). The number of trials can be tuned according to the expected confidence level- the probability that the exact value is within a predefined error margin. In this section, we experimentally extract the number of trials to achieve the statistical significant results with the confidence level= 90\% and error margin= 3\%. 
%figure
\begin{figure*}
\centering
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{images/run-permanent3.png} %, height=5cm
\caption{Permanent Fault: stuck-at-1 and stuck-at-0.}
\label{fig:run_permanent}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{images/run-transient3.png} %, height=5cm
\caption{Transient Fault.}
\label{fig:run_transient}
\end{subfigure}
\caption{{\color{black}Analyzing the number of required trials to achieve statistically significant results. In these charts, a single-bit fault is investigated. The x-axis represents the number of trials. The y-axis represents the aggregated average error rate of the RTL design of the DNN.}}
\label{fig;runs}
\end{figure*}

Experimental results are shown in Figure \ref{fig;runs}, in terms of the aggregated average error rate of the DNN in the y-axis and the number of trials in the x-axis. As it can be seen, with 421, 391, and 31 trials and with standard deviations of 0.33\%, 0.23\%, and 0.002\% for stuck-at-1, stuck-at-0, and transient cases, respectively, our predefined targets (confidence level= 90\% with error margin= 3\%) are satisfied. Note that as mentioned earlier, the total number of permutations to inject a transient fault is significantly more than the case of a permanent fault, 7890772 vs. 4969. However, we observe that to achieve a certain level of confidence, we need considerably less number of trials, in the transient against permanent case. We believe that is the consequence of the momentary nature of transient faults, where a transient bit corruption does not affect the overall DNN output considerably. 

In this paper, we repeat fault characterization and mitigation experiments 421, 391, and 31 times (each time with a different randomly-generated fault), for stuck-at-1, stuck-at-0, and transient cases, respectively. The final results on the classification error are reported as the average of all trials.




==> chapters/5-examples.tex <==
\section{Illustrating the methodology}
\label{sec:examples}
In Section \ref{sec:example1}, we elaborate how our RTL design of the DNN works and in Section \ref{sec:example2}, we show how injected faults propagate through the design.
\subsection{How does the RTL Design of the DNN Model Work?}
\label{sec:example1}
Figure \ref{fig:pipe_example} shows the execution model of an illustrative DNN. For convenience, corresponding information is shown in different parts, as below: 
\begin{itemize}
\item \encircle{1} The illustrative DNN is a small 3-layer network with 4, 2 and, 1 neurons in the input, hidden, and output layers, respectively. 
\item \encircle{2} Weights of different DNN layers are kept in two on-chip memories, to enable the parallel execution. 
\item \encircle{3} and \encircle{4} To perform the classification, two matrix multiplications are required: $layer_0$ for the input and hidden layers, and $layer_1$ for the hidden and output layers. The activation function is logsig. 
\item \encircle{5} The number of $PE$s is 2, which corresponds to two operations per cycle. 
\item \encircle{6} and \encircle{7} The cycle-accurate data-flow execution steps to multiply matrices in $layer_0$ and $layer_1$ are shown. As explained earlier, three types of registers are exploited to accommodate various types of data (in this example, 2 from each type). Among them, \textit{IR}s and \textit{WR}s are inputs of multipliers and results are loaded into \textit{IMRs}.
\end{itemize}

Considering the large size of matrices, the available hardware, the number of $PE$s= 2, is not large enough to perform all computations in a single cycle (in general, this limitation exists for large matrix multiplications on hardware \cite{dou200564}). As a result, the matrix multiplications take multiple cycles (five, in this example) to complete, i.e. four and one cycles for the matrix multiplication of $layer_0$ and $layer_1$, as detailed cycle-by-cycle in the part \encircle{6} and \encircle{7}, respectively. Note that the activation function (logsig) is a combinational circuit that does not incur any additional clock cycle. For convenience, the content of various registers are shown in each cycle of the execution with different colors. Finally, at the end of the 5th cycle, the output of the classifier is calculated as 0.62. 
\subsection{How do Faults Propagate?}
\label{sec:example2}
Figure \ref{fig:pipe_fault} illustrates the propagation of faults (stuck-at-0, stuck-at-1, and transient) corresponding to the illustrative DNN of Figure \ref{fig:pipe_example}. All registers of the design (\textit{IR}s, \textit{WR}s, and \textit{IMR}s) can be potentially affected by faults. For the sake of clarity in explanations, the example only shows the propagation of a single fault in the \underline{sign-bit} of \underline{$WR_0$}. Also, as we explain in Section \ref{sec1}, our experimental results are based on two's complement data representation. However, for convenience, in this example we assume that data are represented in one's complement model, in which a sign-bit flip converts the original value of the corresponding register to its logically reversed value. For example, a sign-bit flip of +0.1 converts it to -0.1.

Permanent faults remain during the entire execution time of $layer_0$ and $layer_1$, five cycles in this example. A permanent fault causes data corruptions for all data items that are stored in the faulty register during the entire execution cycles. In contrast, a transient fault is manifests for a few cycles at most, and in this example, only in the first cycle of $layer_0$ computation. The affected data items as a consequence of the injected fault are surrounded by gray-scale boxes in Figure \ref{fig:pipe_fault}. The fault propagation among layers is also {\color{black}\underline{highlighted}}, which finally leads to a different classification output, in comparison to the fault-free illustrative DNN of Figure \ref{fig:pipe_example}.   


%figure
\begin{figure*}
\centering
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\linewidth]{images/example-pipeline.pdf} %, height=5cm
\caption{An example of execution model of the classification on our RTL model of DNN.}
\label{fig:pipe_example}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\linewidth]{images/fault_example.pdf} %, height=5cm
\caption{An example of the propagation of fault in the illustrative DNN of Figure \ref{fig:pipe_example}. Data items that are \textbf{affected} by faults are surrounded by gray-scale boxes, among them any {\color{red}\underline{bit flips}} are highlighted. Furthermore, {\color{blue}\underline{propagation of faults}} through DNN layers is highlighted.}
\label{fig:pipe_fault}
\end{subfigure}
\caption{Two examples to illustrate the methodology.}
\end{figure*} 


==> chapters/6-baseline_configuration.tex <==
\section{baseline setup and vulnerability aspects}
\label{sec:baseline}
We introduce the baseline setup of the design in Section \ref{sec1} and analyze its overall vulnerability aspects in Section \ref{sec2}. Note that the study on the characterization of the fault behavior in Section \ref{sec:vul} is based on modifications of the baseline setup.
\subsection{Baseline Setup of the RTL Design of the DNN Model}
\label{sec1}
The baseline setup of the design is summarized in Table \ref{default_configl} and described next.
\subsubsection{\textbf{DNN Configuration}}
\label{secB:3}
We use the MNIST dataset \cite{lecun1998gradient} of handwritten digits, in which each image is composed of 784 8-bit pixels. The training phase of the DNN is performed off-line using 60000 training images, by a MATLAB implementation of the network.\footnote{To achieve a significant accuracy, we train the DNN using Autoencoders \cite{autoencoder}.} For the classification, we first export weights and biases of the trained DNN, initialize on-chip memories of our RTL design, and then start streaming input images at 512 bits/cycle from the off-chip memory. The baseline adopted DNN is fully connected and composed of three layers. The size of the input, hidden and output layers is 784, 128, and 10, respectively. Thus, there are two matrix multipliers: $layer_0$ for multiplying the input and hidden layers and $layer_1$ for multiplying the hidden and output layers. The total number of clock cycles to classify an image can be calculated as $T = \frac{784*128 + 128*10}{64} = 1588$ cycles, as formulated in Equation \ref{T}. Also, the activation function is \textit{logsig}, which non-linearly bounds data in the [0, 1] range. With respect to the nonlinear structure of the \textit{logsig}, we use a piece-wise linear implementation in our HLS development. The output of the matrix multiplication in the last layer of the DNN, $layer_1$, is a vector of 10 numbers and the final output is generated after a softmax function is applied on them. At the end, the classification error is computed as the percentage of missclassified images. 

\subsubsection{\textbf{Hardware Platform}} 
\label{secB:2}
In this paper, we work on an RTL design of a DNN. Consequently, with an HLS approach, our hardware units (off/on-chip memories and $PE$s) are Bluespec modules. 
%Hence, we use BRAM cores as on-chip memories with a single-cycle latency, RegFile as off-chip memory with a simulated 512 bits/cycle bandwidth, and FixedPoint multiplier-adder elements as our computation modules \cite{bluespec}.
%However, with the overall architecture in the mind, we parameterized the number of parallel elements ($P$), or the number of on-chip memories and multiplier-adder units, to be able to investigate its impact on the overall vulnerability. 
In the baseline setup, the number of $PE$s is set to 64 that implies that 64 operations can be performed, simultaneously. Accordingly, number of \textit{IR}s, \textit{WR}s, and \textit{IMR}s are 64, 64, and 127, respectively, to cope with generated/loaded data during the computation. With respect to Equation \ref{S}, the total number of bits that can be potentially affected by faults is: $S= (64*16)+ (64*16)+ (127*23)= 4969$.   %\footnote{Our post-placement and routing reports on the zedboard 7000 fabric show that the flip-flop (FF) usage is 13.3\%, which are mainly used for registers of the design. LUT usage is 46.6\%, which are used as computation units (multipliers and adders). Also, the BRAM utilization is (53.3\%), as 64 out of total 120 are used.}

\subsubsection{\textbf{Data Representation Model}}
\label{secB:1}
We use low-precision fixed-point data representation. For this aim, we leverage fixed-point libraries of Bluespec, which inherently represents negative numbers in two's complement format. Fixed-point data model performs well-enough for DNN classifiers that leads to low-power performance \cite{reagen2016minerva}.
%\footnote{An estimation of total power consumption of our RTL model on Xilinx Vivado tool is 2.6 watts (dynamic: 2.3 watts, static: 0.3 watts). It is on average, an order of magnitude less than recent GPU \cite{yazdanbakhsh2015neural} and CPU implementations \cite{bastien2012theano} of DNN, which are commonly using the floating-point data model.}. 
Accordingly, we use the minimum required number of sign, digit, and fraction bits for various types of registers. To find the minimum bit-width without affecting the DNN accuracy, we first run a fault-free classifier on the MNIST benchmark \cite{lecun1998gradient}. We observe that \textit{IR}s do not need sign and digit bits and having only the fraction component is good enough, since they are used to accommodate either input data (in $layer_0$) or outputs of the $layer_0$ (in $layer_1$), which in both cases are in the [0,1] range. As in the $layer_0$, we use a normalized version of input data in the [0,1] range and also, in the $layer_1$ data are loaded from the \textit{logsig} activation function of $layer_0$. Additionally, we observe that \textit{WR}s needs at least 1, 4, and 11 bit(s) and  \textit{IMR}s needs at least 1, 6, and 16 bit(s) for the sign, digit, and fraction components, respectively. Thus, the total bit-width (sum of the sign, digit, and fraction bit-widths) of \textit{IR}s, \textit{WR}s, and \textit{IMR}s are set to 16, 16, and 23, respectively.


%table
\begin{table}[]
\centering
\caption{The baseline setup of the RTL design of the DNN.}
\label{default_configl}
\begin{tabular}{|l|l|l|}
\hline
DNN Configuration & Hardware Platform & Data Representation Model \\ \hline \hline
\begin{tabular}[c]{@{}l@{}}size: 784-128-10\\ activation function: logsig\\ benchmark: MNIST\\ \#input data items: 10000\end{tabular}  & \begin{tabular}[c]{@{}l@{}}number of $PE$s: 64\\ number of \textit{IR}s: 64\\ number of \textit{WR}s: 64\\number of \textit{IMR}s: 127\end{tabular} &  \begin{tabular}[c]{@{}l@{}}fixed-point (two's complement)\\size of \textit{IR}s: 16-bits   (\textit{s}: 0, \textit{d}: 0, \textit{f}: 16)\tnote{1}\\size of \textit{WR}s: 16-bits (\textit{s}: 1, \textit{d}: 4, \textit{f}: 11)\\size of \textit{IMR}s: 23-bits (\textit{s}: 1, \textit{d}: 6, \textit{f}: 16)\end{tabular}
 \\ \hline
\end{tabular}
\begin{tablenotes}
    \item[1] In this table, \textit{s}, \textit{d}, and \textit{f} refer to bit-width of sign, digit, and fraction components, respectively.
  \end{tablenotes}
\label{table:precision}
\end{table}
 


\subsection{Fault Propagation Analysis} 
\label{sec2}


In this section, we analyze the propagation of faults through the DNN, by injecting individual types of faults (stuck-at-0, stuck-at-1, and transient) within all \underline{non-sign} bits of all registers (\textit{IR}s, \textit{WR}s, and \textit{IMR}s). The impact of sign-bit faults is discussed in Section \ref{sec:mitigation}. Experimental results with the baseline setup are shown in Figure \ref{fig:fault_default}. Also, to verify results, in addition to the MNIST, we repeat these experiments using another common DNN benchmark, Forest \cite{Krizhevsky2009}. The x-axis represents the number of injected faults per input image, which varies from 0, the original non-faulty DNN with only an inherent classification error, to 22, the case in which all non-sign bits of the corresponding register are corrupted. Note that the maximum size of registers is 23-bits, which means that we can inject a maximum of 22 faults in non-sign bits. We observe that:
\begin{itemize}
\item Permanent faults cause higher errors than transient, as expected. This is due to the fact that permanent faults stuck for the whole period of the computation (for instance, $T$= 1588 for the baseline setup of the MNIST), while transient faults are manifest for one cycle.   
\item Stuck-at-1 faults cause higher errors than stuck-at-0. We observe that our benchmarks are near-zero sparse dataset, resulting in more zero than one bits in the registers of the RTL design (4.5X on average), as seen in Figure \ref{fig:hist2} for the MNIST (and similar for Forest). Consequently, stuck-at-1 faults exhibit a significantly higher impact on the DNN accuracy than stuck-at-0 faults.
\end{itemize}

Although, the inherent classification error in Forest (34.5\%) is higher than the MNIST (2.9\%), we do not observe a significant difference in the behavior of the vulnerability experiments, as both cope with near-zero data. Thus, for convenience we present rest of results only for the MNIST benchmark.    


\begin{figure}
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/overall0.png} %, height=5cm
\caption{Stuck-at-0}
\label{fig:fault_default_0}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/overall1.png} %, height=5cm
\caption{Stuck-at-1}
\label{fig:fault_default_1}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/overall2.png} %, height=5cm
\caption{Transient}
\label{fig:fault_default_2}
\end{subfigure}
\caption{Impact of faults in the DNN accuracy with the baseline setup of the design for MNIST and Forest.}
\label{fig:fault_default}
\end{figure} 

%figure
\begin{figure}
\centering
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{images/his0.png} %, height=5cm
\caption{The number of zero and one bits of Intermediate Registers (\textit{IMR}s) and Weight Registers (\textit{WR}s).}
\label{fig:hist2}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\centering
\includegraphics[width=\linewidth]{images/his1.png} %, height=5cm
\caption{A histogram of values of Input Registers (\textit{IR}s).}
\label{fig:histogram_0}
\end{subfigure}
%\includegraphics[width=8cm]{images/histogram_2.png} %, height=5cm
\caption{Histograms to show the sparsity of data (input, weights, intermediate) for the MNIST benchmark, used to justify some of our experimental results: \textbf{a)} why stuck-at-1 faults cause higher classification errors than stuck-at-0 faults. \textbf{b)} why \textit{IMR}s are more vulnerable than \textit{WR}s.}
\label{fig:hist}
\end{figure} 

==> chapters/8-verification.tex <==
{\color{black}\section{Verification of Experimental Results of the Fault Characterization}
\label{sec:verification} 
In Sections \ref{sec:baseline} and \ref{sec:vul}, we present and discuss the resilience aspects of DNN RTL on MNIST benchmark dataset \cite{lecun1998gradient}. However, to verify our observations and conclusions, we repeat the fault injection methodology, on another common benchmark, Forest \cite{Krizhevsky2009}. By this experiment, we can infer how much our results are generic and benchmark-free. Toward this goal, as usual, we train DNN in MATLAB on Forest dataset, extract weights and biases, load them into on-chip memories of our RTL DNN, and finally run the classifier, while randomly-generated faults are injected. 

Forest consists of 581012 records of forest cover types that are classified into 7 classes. Among them, 11340, 3780, and 565892 are used as training, validation, and classification, respectively. Each record is composed of 54 fields with various data types, e.g., integer, binary. Accordingly, to run Forest benchmark, DNN needs 54 and 7 neurons in the input and output layers, respectively. In this section, our experiments are on a 3-layer DNN with the size of 54-1024-7. It is compared against a 3-layer DNN with 1024 neurons in the hidden layer on MNIST, in short with the size of 784-1024-10. Due to their relatively various sizes of input and output layers, it can be computed that $T_{Forest}= 1024$ vs. $T_{MNIST}= 12704$, with respect to Equation \ref{T}. Experimental results of the vulnerability analysis on Forest vs. MNIST benchmarks are shown in Figures \ref{fig:s0}, \ref{fig:s1}, and \ref{fig:t}, for stuck-at-0, stuck-at-1, and transient cases, respectively. For convenience, in this section, we inject faults in non-sign bits of \textit{WR}s, thus, the number of faults in x-axis varies from 0 to 15. We observe that:
\begin{itemize}
\item Inherent classification error in Forest is higher than MNIST: We observe 34.5\% error on Forest vs. 1.8\% on MNIST. This is close to the nominal error for other implementations \cite{reagen2016minerva}. 
\item Permanent faults lead to higher classification error in MNIST vs. Forest: As noted earlier, $T_{Forest}= 1024$ vs. $T_{MNIST}= 12704$, which in turn, causes higher error in MNIST vs. Forest, on average by 1.6X, as permanent faults stuck for the whole classification time.
\end{itemize}

Other overall behaviors of fault study are the similar for Forest and MNIST, e.g., higher errors as a consequence of stuck-at-1 vs. stuck-at-0 and higher errors as a consequence of permanent vs. transient faults. In short, we do not observe a significant difference on the behavior of vulnerability experiments on Forest vs. MNIST, as both benchmarks cause sparse computations with near-zero input, weights, and intermediate data.


\begin{figure*}
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/mnist-forest0.png} %, height=5cm
\caption{stuck-at-0}
\label{fig:s0}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/mnist-forest1.png} %, height=5cm
\caption{stuck-at-1}
\label{fig:s1}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\includegraphics[width=\linewidth]{images/mnist-forest2.png} %, height=5cm
\caption{transient}
\label{fig:t}
\end{subfigure}
\caption{{\color{black}Overall vulnerability of the design on various benchmarks, MNIST vs. Forest.}}
\label{fig:mnistcifar}
\end{figure*}

}

==> chapters/keyparam-bak.tex <==
\subsubsection{Key Parameters of Vulnerability Analysis (Number of Faults and Number of Accesses)}
The vulnerability of a system highly depends on the architecture of the underlying hardware, the inherent specifications of the application, the representation model of data, etc. However, in \cite{Yu2014} it is shown that in general, two parameters play crucial roles in the system vulnerability: the number of faults ($N_{faults}$) and the number of hardware accesses to a faulty component of the system ($N_a$). In this section, we demonstrate these two parameters for our design, as below, whereas they will be used in the experimental section to explain results. 
\begin{itemize}
\item \textbf{The number of faults ($N_{faults}$):} This parameter can be computed as a linear function of fault rate ($FR$), the execution time ($T$), and the total number of bits ($S$), as Equation (1), where, \textbf{\textit{i)}} $FR$ indicates the rate of failure per bit and per cycle. In a below safe-voltage design, $FR$ is the consequence of different voltage scales, which can be modeled either by HSpice simulations \cite{reagen2016minerva} or an actual experiment \cite{Ganapathy2017}. \textbf{\textit{ii)}} $T$ represents the total number of cycles to classify an input image, in our system. As it is shown in Equation (2), $T$ can be computed as a function of total number of multiply-add operations, which equals to the sum of the operations of all the required matrices multiplications ($\sum_{i=0}^{N_l-2} {|L_i| * |L_{i+1}|}$). In this formulation, we assume that DNN has $N_l$ layers in total, i.e., $\{L_0, L_1, ..., L_{N_l-1}\}$, where $L_0$ is the input layer, $L_{N_l-1}$ is the output layer, and the rest are hidden layers of DNN. $|L_i|$ indicates the size of the layer $i$, which equals to the number of neurons. Also, $T$ is indirectly in relation with the number of parallel elements ($P$), as an architecture-dependent parameter. Because $P$ parallel elements (storage and processing) lead to a performance of $P$ operations (multiplier/adder) per cycle. And, \textbf{\textit{iii)}} $S$ represents the total number of bits of the design, which can be potentially corrupted. With respect to the RTL model of our system, where we inject faults in registers of the design, we can compute $S$ as the aggregation of the "number of the registers ($numReg$) multiplied by number of the bits ($sizeReg$)", as Equation (3). Different types of registers and their specifications are introduced in Section 6, for our baseline design. 

To get our results, we present experiments in terms of number of faults ($N_{faults}$), which in a given design (with constant $T$ and $S$), is the consequence of the fault rate ($FR$). Accordingly, as we inject faults in a single register, $N_{faults}$ varies from a minimum number (1) to a maximum number (the bit width of the corresponding faulty register).  
\item \textbf{The number of accesses ($N_a$):} $N_a$ indicates the number of data items that are affected by a fault, which is the consequence of the register reuse method that is explained in Section 4.2.4. $N_a$=1 for the case of transient fault, as a transient fault flips a data item for a single cycle, mostly. However, as permanent faults manifest themselves as stuck-at faults for whole the classification time, $N_a$ equals the number of total clock cycles of the classification ($T$), which is already shown in Equation (2). Accordingly, Equation (4) represents values of $N_a$ for different types of faults, individually.
\end{itemize}

%\begin{equation}
%Vulnerability \sim N_{faults} * N_{a}
%\end{equation}
\begin{equation}
N_{faults} = FR * T * S
\end{equation}
\begin{equation}
T = \frac{\sum_{i=0}^{N_l-2} {|L_i| * |L_{i+1}|}}{P}
\end{equation}
\begin{equation}
S = \sum_{i \in RegTypes}{numReg_i * sizeReg_i}
\end{equation}
\begin{equation}
N_a = \Big\{ \begin{tabular}{cc}
T  & permanent\\
1  & transient
\end{tabular}
\end{equation}
